SciDataCopilot: An Agentic Data Preparation Framework for AGI-driven Scientific Discovery

The current landscape of AI for Science (AI4S) is predominantly anchored in large-scale textual corpora, where generative AI systems excel at hypothesis generation, literature search, and multi-modal reasoning. However, a critical bottleneck for accelerating closed-loop scientific discovery remains the utilization of raw experimental data. Characterized by extreme heterogeneity, high specificity, and deep domain expertise requirements, raw data possess neither direct semantic alignment with linguistic representations nor structural homogeneity suitable for a unified embedding space. The disconnect prevents the emerging class of Artificial General Intelligence for Science (AGI4S) from effectively interfacing with the physical reality of experimentation. In this work, we extend the text-centric AI-Ready concept to Scientific AI-Ready data paradigm, explicitly formalizing how scientific data is specified, structured, and composed within a computational workflow. To operationalize this idea, we propose SciDataCopilot, an autonomous agentic framework designed to handle data ingestion, scientific intent parsing, and multi-modal integration in a end-to-end manner. By positioning data readiness as a core operational primitive, the framework provides a principled foundation for reusable, transferable systems, enabling the transition toward experiment-driven scientific general intelligence. Extensive evaluations across three heterogeneous scientific domains show that SciDataCopilot improves efficiency, scalability, and consistency over manual pipelines, with up to 30$\times$ speedup in data preparation.

==> sections/7-author.tex <==
\newpage
\section*{Authors}
\addcontentsline{toc}{section}{Authors}
\label{sec:authors}

\textbf{Co-first Authors}

Jiyong Rao, Yicheng Qiu, Jiahui Zhang, Juntao Deng, Shangquan Sun

\textbf{Contributors}

% ai4neuro
% 伍佳敏，郑启豪，刘棉莘，朱宇
% Jiamin Wu, Qihao Zheng, Mianxin Liu, Yu Zhu,
% % ai4s
% % 零丰华、张铂、张文龙、唐诗翔、董楠卿、李玉强、王潚崧、周东展
% Fenghua Ling, Hao Chen, Bo Zhang, Wenlong Zhang, Shixiang Tang, Nanqing Dong, Yuqiang Li, Xiaosong Wang, Dongzhan Zhou,
% % others
% % 何聪辉、王广宇、吴郦军，邵婧、汪旭鸿
% Conghui He, Guangyu Wang, Lijun Wu, Jing Shao, Xuhong Wang,
% %
% Wanli Ouyang

% earth-life-material
Fenghua Ling, Hao Chen, Nanqing Dong, Zhangyang Gao, Siqi Sun, Yuqiang Li, Dongzhan Zhou, 
Guangyu Wang, Lijun Wu, Conghui He, Xuhong Wang, Jing Shao, 
% neuro
Xiang Liu, Yu Zhu, Mianxin Liu, Qihao Zheng, Yinghui Zhang, Jiamin Wu,
% data-safety
Xiaosong Wang, Shixiang Tang, Wenlong Zhang, Bo Zhang, 
%
Wanli Ouyang

\textbf{Corresponding Authors}

Runkai Zhao, Chunfeng Song, Lei Bai, Chi Zhang

\textbf{Project Lead}

Chi Zhang (zhangchi2@pjlab.org.cn)

\textbf{Main Affiliations}

Shanghai Artificial Intelligence Laboratory

==> sections/codes/code_00.tex <==
% [0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0]% [0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0][0]
\begin{tcolorbox}[
    breakable,
    title=Example of Dry Experiment in Astronomy,
    colback=LighterGray,
    colframe=DeepPurple,
    colbacktitle=DeepPurple,
    coltitle=White,
]
\textbf{\emph{\textcolor{DeepPurple}{Background}}}


The Zwicky Transient Facility (ZTF) is an advanced optical time-domain sky survey utilizing the Palomar 48-inch Schmidt telescope equipped with a custom wide-field CCD camera. This camera covers a 47.7 square degree field of view with 16 large-format CCDs, enabling a survey speed over an order of magnitude faster than its predecessor. The system achieves a median image quality of approximately 2.0 arcseconds full-width at half-maximum (FWHM) across g, r, and i bands, with typical 5-sigma limiting magnitudes near 20.8 (g), 20.6 (r), and 19.9 (i) in 30-second exposures, improving under dark-sky conditions.

The optical design addresses the Schmidt telescopes curved focal surface through a combination of a modified Schmidt corrector, a meniscus dewar window, faceted cold plate mounting, and individual field flattener lenses above each CCD. The cameras cryostat and readout electronics are optimized for minimal beam obstruction and rapid 8.2-second readout with low noise (~10 electrons median). A robotic observing system and scheduler maximize volumetric survey speed by selecting fields on a fixed grid with minimal dithering, enabling efficient coverage of the Northern sky and Galactic plane.

ZTFs data system performs near-real-time image processing, including bias subtraction, flat-fielding, astrometric and photometric calibration, and image differencing using the ZOGY algorithm to detect transient and variable sources. Alerts containing rich contextual information and machine-learning-based Real-Bogus scores are distributed via a scalable streaming system to community brokers. The system also supports solar system science by detecting both point-like and streaked moving objects, linking detections into orbits, and reporting to the Minor Planet Center.

Early scientific results demonstrate ZTFs capability to discover and classify supernovae, including young Type II events, and to conduct rapid follow-up of multi-messenger triggers such as neutrinos and gamma-ray bursts. The facility also enables studies of variable stars, exemplified by light curves of Be stars and RR Lyrae, and solar system objects, including near-Earth asteroids, asteroid rotation periods, comet activity, and Centaur outbursts.

ZTFs public surveys include a three-day cadence Northern Sky Survey and a nightly Galactic Plane Survey, with observations typically taken twice per night in g and r bands. The surveys moderate depth and high cadence complement future facilities by providing early discovery and characterization of bright transients accessible to moderate-aperture telescopes. ZTF serves as a pathfinder for next-generation surveys, offering a prototype alert stream and extensive time-domain data products to the astronomical community.

\textbf{\emph{\textcolor{DeepPurple}{Data Code}}}

\begin{lstlisting}
#!/usr/bin/env python3
# -*- coding: utf-8 -*-
"""
Paper: The Zwicky Transient Facility: System Overview, Performance, and First Results
Authors: Eric C. Bellm, Shrinivas R. Kulkarni, Matthew J. Graham, et al.
Year: 2019

This script generates synthetic asteroid light curve data based on the descriptions
in Section 6.4.2 of the paper.

Python Version: 3.10.12
"""

import sys
assert sys.version_info >= (3, 10), "This code requires Python 3.10 or higher"

# Dependencies
# pip install numpy==1.24.3 pandas==2.0.3

import numpy as np
import pandas as pd
from pathlib import Path
from typing import Tuple

# Global constants
DATA_DIR = Path("data")
DEFAULT_FILE_PATH = DATA_DIR / "asteroid_light_curve.csv"
RANDOM_SEED = 42 # Ensure reproducible results

def generate_asteroid_light_curve(
    file_path: str,
    n_points: int = 150,
    period_hr: float = 2.25,
    amplitude: float = 0.2,
    mag_range: Tuple[float, float] = (17.8, 18.2),
    noise_level: float = 0.03
) -> None:
    """
    Generates a synthetic asteroid light curve and saves it to a CSV file.
    The light curve is modeled as a simple cosine function with added Gaussian noise.
    This mimics the data for an asteroid like (11014) Svatopluk in Figure 10(a).

    Tag: [Data download]

    Args:
        file_path (str): The path to save the output CSV file.
        n_points (int): The number of data points to generate.
        period_hr (float): The rotation period of the asteroid in hours.
        amplitude (float): The amplitude of the light curve variation in magnitudes.
        mag_range (Tuple[float, float]): The approximate magnitude range of the asteroid.
        noise_level (float): The standard deviation of the Gaussian noise to add to the magnitudes.

    Returns:
        None

    Examples:
        >>> Path("data").mkdir(exist_ok=True)
        >>> file_path = "data/test_light_curve.csv"
        >>> generate_asteroid_light_curve(file_path, n_points=50)
        >>> import pandas as pd
        >>> df = pd.read_csv(file_path)
        >>> print(df.shape)
        (50, 3)
    """
    # Set random seed to ensure reproducibility
    np.random.seed(0+RANDOM_SEED)

    # Generate unevenly sampled time points to simulate real observations
    # Observation time span is about 4 hours
    observation_span_hr = period_hr * 1.8
    times = np.sort(np.random.rand(n_points) * observation_span_hr)

    # Calculate the baseline magnitude of the light curve
    base_magnitude = np.mean(mag_range)

    # Use cosine function to simulate asteroid brightness variation
    # Multiply by 2 because a full rotation period usually contains two peaks and two troughs
    magnitudes_true = base_magnitude - amplitude * np.cos(2 * np.pi * times / period_hr * 2)

    # Add Gaussian noise to the observed data
    noise = np.random.normal(0, noise_level, n_points)
    magnitudes_obs = magnitudes_true + noise

    # Generate error for each data point, related to noise level
    errors = np.random.normal(noise_level, noise_level / 4, n_points)
    errors = np.maximum(errors, noise_level / 2) # Ensure errors are not too small

    # Create a DataFrame to store the data
    df = pd.DataFrame({
        'time_hr': times,
        'magnitude': magnitudes_obs,
        'error': errors
    })

    # Save to CSV file
    df.to_csv(file_path, index=False)
    print(f"Successfully generated synthetic light curve data and saved to: {file_path}")


if __name__ == "__main__":
    # Ensure data directory exists
    DATA_DIR.mkdir(exist_ok=True)

    # Generate simulated data
    generate_asteroid_light_curve(
        file_path=str(DEFAULT_FILE_PATH),
        n_points=150,
        period_hr=2.25, # Asteroid period corresponding to Figure 10(a)
        amplitude=0.15, # Amplitude
        mag_range=(17.8, 18.1), # Magnitude range
        noise_level=0.02 # Noise level
    )
\end{lstlisting}

\textbf{\emph{\textcolor{DeepPurple}{Main Code with Incomplete Functions}}}

\begin{lstlisting}
#!/usr/bin/env python3
# -*- coding: utf-8 -*-
"""
Paper: The Zwicky Transient Facility: System Overview, Performance, and First Results
Authors: Eric C. Bellm, Shrinivas R. Kulkarni, Matthew J. Graham, et al.
Year: 2019

This script implements the asteroid light curve analysis from Section 6.4.2.
It determines the rotation period of an asteroid from its light curve using
a Lomb-Scargle periodogram and Fourier series fitting.

Python Version: 3.10.12
"""

import sys

assert sys.version_info >= (3, 10), "This code requires Python 3.10 or higher"

# Dependencies
# pip install numpy==1.24.3 pandas==2.0.3 scipy==1.10.1

import numpy as np
import pandas as pd
from scipy.signal import lombscargle
from typing import Tuple
from pathlib import Path

# Global constants
DATA_FILE_PATH = "data/asteroid_light_curve.csv"
# Order of Fourier series, the paper mentions second-order Fourier series
FOURIER_N_TERMS = 2
# Numerical stability constant
EPSILON = 1e-9


def load_light_curve_data(file_path: str) -> pd.DataFrame:
    """
    Loads asteroid light curve data from a CSV file.

    Tag: [Data loading]

    Args:
        file_path (str): The path to the CSV file.

    Returns:
        pd.DataFrame: A DataFrame containing the light curve data with
                      columns 'time_hr', 'magnitude', and 'error'.

    Examples:
        >>> Path("data").mkdir(exist_ok=True)
        >>> data = {'time_hr': [0, 1], 'magnitude': [18.0, 18.1], 'error': [0.01, 0.01]}
        >>> df = pd.DataFrame(data)
        >>> df.to_csv("data/dummy.csv", index=False)
        >>> loaded_df = load_light_curve_data("data/dummy.csv")
        >>> print(loaded_df.shape)
        (2, 3)
    """
    try:
        return pd.read_csv(file_path)
    except FileNotFoundError:
        print(f"Error: Data file not found at '{file_path}'")
        print("Please run 'data.py' first to generate the data file.")
        sys.exit(1)


def calculate_lomb_scargle_periodogram(
        times: np.ndarray,
        magnitudes: np.ndarray,
        min_period: float = 0.5,
        max_period: float = 5.0,
        num_periods: int = 10000
) -> Tuple[np.ndarray, np.ndarray]:
    """
    Calculates the Lomb-Scargle periodogram for unevenly sampled data.

    Tag: [Numerical calculation]

    Args:
        times (np.ndarray): Array of time points.
        magnitudes (np.ndarray): Array of magnitude measurements.
        min_period (float): The minimum period to test.
        max_period (float): The maximum period to test.
        num_periods (int): The number of period points to evaluate.

    Returns:
        Tuple[np.ndarray, np.ndarray]: A tuple containing the periods tested
                                       and the corresponding periodogram power.

    Examples:
        >>> times = np.linspace(0, 4, 50)
        >>> magnitudes = 18 + 0.1 * np.sin(2 * np.pi * times / 2.0)
        >>> periods, power = calculate_lomb_scargle_periodogram(times, magnitudes)
        >>> print(periods.shape, power.shape)
        (10000,) (10000,)
    """
    pass # [Please complete the code]


def find_best_period_from_periodogram(
        periods: np.ndarray,
        power: np.ndarray
) -> float:
    """
    Finds the period corresponding to the highest power in the periodogram.

    Tag: [Numerical calculation]

    Args:
        periods (np.ndarray): Array of periods.
        power (np.ndarray): Array of periodogram powers.

    Returns:
        float: The period with the highest power.

    Examples:
        >>> periods = np.array([1.0, 2.0, 3.0])
        >>> power = np.array([0.1, 0.8, 0.2])
        >>> best_period = find_best_period_from_periodogram(periods, power)
        >>> print(best_period)
        2.0
    """
    pass # [Please complete the code]


def build_fourier_design_matrix(
        times: np.ndarray,
        period: float,
        n_terms: int
) -> np.ndarray:
    """
    Builds the design matrix for a Fourier series linear least-squares fit.

    Tag: [Predictive modeling]

    Args:
        times (np.ndarray): Array of time points.
        period (float): The fundamental period of the Fourier series.
        n_terms (int): The number of Fourier terms (harmonics) to include.

    Returns:
        np.ndarray: The design matrix for the fit.

    Examples:
        >>> times = np.array([0, 1, 2])
        >>> period = 4.0
        >>> n_terms = 1
        >>> matrix = build_fourier_design_matrix(times, period, n_terms)
        >>> print(matrix.shape)
        (3, 3)
    """
    # Fundamental frequency
    omega = 2 * np.pi / (period + EPSILON)
    # Initialize a column vector for the constant term
    design_matrix = [np.ones_like(times)]
    # Loop to add sin and cos terms for each order
    for i in range(1, n_terms + 1):
        design_matrix.append(np.sin(i * omega * times))
        design_matrix.append(np.cos(i * omega * times))
    return np.vstack(design_matrix).T


def fit_fourier_model(
        design_matrix: np.ndarray,
        magnitudes: np.ndarray,
        errors: np.ndarray
) -> np.ndarray:
    """
    Fits a Fourier model using weighted linear least squares.

    Tag: [Predictive modeling]

    Args:
        design_matrix (np.ndarray): The design matrix from build_fourier_design_matrix.
        magnitudes (np.ndarray): Array of magnitude measurements.
        errors (np.ndarray): Array of measurement errors for weighting.

    Returns:
        np.ndarray: The array of fitted Fourier coefficients.

    Examples:
        >>> times = np.linspace(0, 4, 10)
        >>> period = 2.0
        >>> magnitudes = np.sin(2 * np.pi * times / period)
        >>> errors = np.full_like(magnitudes, 0.1)
        >>> matrix = build_fourier_design_matrix(times, period, 1)
        >>> coeffs = fit_fourier_model(matrix, magnitudes, errors)
        >>> print(len(coeffs))
        3
    """
    # Use errors for weighting
    weights = 1.0 / (errors + EPSILON)
    weighted_matrix = design_matrix * weights[:, np.newaxis]
    weighted_magnitudes = magnitudes * weights

    # Solve using least squares
    coeffs, _, _, _ = np.linalg.lstsq(weighted_matrix, weighted_magnitudes, rcond=None)
    return coeffs


def evaluate_fourier_model(
        design_matrix: np.ndarray,
        coeffs: np.ndarray
) -> np.ndarray:
    """
    Evaluates the Fourier model at given time points.

    Tag: [Numerical calculation]

    Args:
        design_matrix (np.ndarray): The design matrix.
        coeffs (np.ndarray): The fitted Fourier coefficients.

    Returns:
        np.ndarray: The predicted magnitudes from the model.

    Examples:
        >>> times = np.array([0, 1, 2])
        >>> period = 4.0
        >>> n_terms = 1
        >>> matrix = build_fourier_design_matrix(times, period, n_terms)
        >>> coeffs = np.array([18.0, 0.1, 0.0])
        >>> model_mags = evaluate_fourier_model(matrix, coeffs)
        >>> print(model_mags.shape)
        (3,)
    """
    return np.dot(design_matrix, coeffs)


def calculate_reduced_chi_squared(
        observed: np.ndarray,
        expected: np.ndarray,
        errors: np.ndarray,
        num_fit_params: int
) -> float:
    """
    Calculates the reduced chi-squared statistic for a fit.

    Tag: [Metric calculation]

    Args:
        observed (np.ndarray): The observed data values.
        expected (np.ndarray): The model's expected values.
        errors (np.ndarray): The errors on the observed values.
        num_fit_params (int): The number of free parameters in the model.

    Returns:
        float: The reduced chi-squared value.

    Examples:
        >>> obs = np.array([1, 2, 3])
        >>> exp = np.array([1.1, 2.2, 2.9])
        >>> err = np.array([0.2, 0.2, 0.2])
        >>> r_chi2 = calculate_reduced_chi_squared(obs, exp, err, 1)
        >>> print(f"{r_chi2:.2f}")
        1.25
    """
    # Calculate chi-squared value
    chi_squared = np.sum(((observed - expected) / (errors + EPSILON)) ** 2)
    # Calculate degrees of freedom
    degrees_of_freedom = len(observed) - num_fit_params
    # Avoid division by zero
    if degrees_of_freedom <= 0:
        return np.inf
    return chi_squared / degrees_of_freedom


if __name__ == "__main__":
    print("--- ZTF Asteroid Light Curve Analysis ---")

    # 1. Load data
    print(f"\n[1/4] Loading light curve data from '{DATA_FILE_PATH}'...")
    light_curve_df = load_light_curve_data(DATA_FILE_PATH)
    times = light_curve_df['time_hr'].values
    magnitudes = light_curve_df['magnitude'].values
    errors = light_curve_df['error'].values
    print(f"Successfully loaded {len(times)} data points.")

    # 2. Calculate Lomb-Scargle periodogram
    print("\n[2/4] Calculating periodogram using Lomb-Scargle method...")
    # Set a reasonable period search range
    min_p = 0.5  # hours
    max_p = (times.max() - times.min())  # observation span as max period
    periods, power = calculate_lomb_scargle_periodogram(times, magnitudes, min_period=min_p, max_period=max_p)
    best_period = find_best_period_from_periodogram(periods, power)
    print(f"Periodogram analysis complete. Most likely light curve period is: {best_period:.4f} hours.")

    # 3. Fit Fourier series model
    print(f"\n[3/4] Fitting {FOURIER_N_TERMS}-order Fourier series using found period {best_period:.4f} hours...")
    design_matrix = build_fourier_design_matrix(times, best_period, FOURIER_N_TERMS)
    fourier_coeffs = fit_fourier_model(design_matrix, magnitudes, errors)
    model_magnitudes = evaluate_fourier_model(design_matrix, fourier_coeffs)
    print("Fourier model fitting complete.")
    print(f"Fitted coefficients: {np.round(fourier_coeffs, 4)}")

    # 4. Evaluate goodness of fit
    print("\n[4/4] Evaluating model goodness of fit...")
    num_params = 1 + 2 * FOURIER_N_TERMS  # 1 constant term + n*2 sin/cos terms
    r_chi2 = calculate_reduced_chi_squared(magnitudes, model_magnitudes, errors, num_params)
    print(f"Reduced chi-squared of the model: {r_chi2:.4f}")
    if 0.5 < r_chi2 < 2.0:
        print("This is a reasonable fit.")
    else:
        print("Warning: The fit may be poor or error estimates inaccurate.")

    # Final output
    # The core goal in the paper for finding asteroid rotation period is to obtain the period value
    print("\n--- Analysis Complete ---")
    print("[Final Output]")
    # Since the asteroid rotation causes two peaks in the light curve per rotation,
    # the physical rotation period is twice the light curve period found by Lomb-Scargle
    # This is a common convention in astronomy
    rotation_period = best_period * 2.0
    print(f"{rotation_period:.4f}")
\end{lstlisting}

\textbf{\emph{\textcolor{DeepPurple}{Answer}}}

\begin{lstlisting}
def calculate_lomb_scargle_periodogram(
        times: np.ndarray,
        magnitudes: np.ndarray,
        min_period: float = 0.5,
        max_period: float = 5.0,
        num_periods: int = 10000
) -> Tuple[np.ndarray, np.ndarray]:
    """
    Calculates the Lomb-Scargle periodogram for unevenly sampled data.

    Tag: [Numerical calculation]

    Args:
        times (np.ndarray): Array of time points.
        magnitudes (np.ndarray): Array of magnitude measurements.
        min_period (float): The minimum period to test.
        max_period (float): The maximum period to test.
        num_periods (int): The number of period points to evaluate.

    Returns:
        Tuple[np.ndarray, np.ndarray]: A tuple containing the periods tested
                                       and the corresponding periodogram power.

    Examples:
        >>> times = np.linspace(0, 4, 50)
        >>> magnitudes = 18 + 0.1 * np.sin(2 * np.pi * times / 2.0)
        >>> periods, power = calculate_lomb_scargle_periodogram(times, magnitudes)
        >>> print(periods.shape, power.shape)
        (10000,) (10000,)
    """
    # 1. Define and generate the search range for ordinary frequencies (f = 1/P)
    safe_min_period = max(min_period, EPSILON)
    min_freq = 1.0 / max_period
    max_freq = 1.0 / safe_min_period
    ordinary_frequencies = np.linspace(min_freq, max_freq, num_periods)

    # 2. [Key modification] Convert ordinary frequencies to angular frequencies (omega = 2*pi*f)
    # scipy.signal.lombscargle requires angular frequencies as input
    angular_frequencies = 2 * np.pi * ordinary_frequencies

    # 3. Center magnitude data to remove DC component
    magnitudes_centered = magnitudes - np.mean(magnitudes)

    # 4. Calculate periodogram power using angular frequencies
    power = lombscargle(times, magnitudes_centered, angular_frequencies, normalize=True)

    # 5. Return periods (P = 1/f) corresponding to ordinary frequencies and power
    periods = 1.0 / (ordinary_frequencies + EPSILON)
    return periods, power

def find_best_period_from_periodogram(
        periods: np.ndarray,
        power: np.ndarray
) -> float:
    """
    Finds the period corresponding to the highest power in the periodogram.

    Tag: [Numerical calculation]

    Args:
        periods (np.ndarray): Array of periods.
        power (np.ndarray): Array of periodogram powers.

    Returns:
        float: The period with the highest power.

    Examples:
        >>> periods = np.array([1.0, 2.0, 3.0])
        >>> power = np.array([0.1, 0.8, 0.2])
        >>> best_period = find_best_period_from_periodogram(periods, power)
        >>> print(best_period)
        2.0
    """
    best_period_index = np.argmax(power)
    return periods[best_period_index]
\end{lstlisting}

\end{tcolorbox}
%-----------------------------------------------------------%-----------------------------------------------------------

==> sections/codes/code_01.tex <==
% [1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1]% [1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1][1]
\begin{tcolorbox}[
    breakable,
    title=Example of Dry Experiment in Earth,
    colback=LighterGray,
    colframe=DeepPurple,
    colbacktitle=DeepPurple,
    coltitle=White,
]
\textbf{\emph{\textcolor{DeepPurple}{Background}}}


Surface ozone is a secondary air pollutant formed by photochemical reactions involving carbon monoxide (CO), volatile organic compounds (VOCs), nitrogen oxides (NOx = NO + NO2), and sunlight. It poses significant risks to human health, including respiratory and cardiovascular effects, and damages vegetation by reducing crop yields and ecosystem productivity. While stringent emission controls since the 1990s have reduced ozone pollution in many Western regions, rapid industrialization and urbanization in East Asia, particularly China, have led to increasing ozone precursor emissions and elevated surface ozone levels.

Recent nationwide monitoring in China, initiated around 2013, reveals that although median ozone concentrations during the warm season (AprilSeptember) are comparable to those in industrialized regions such as Japan, South Korea, Europe, and the United States, the frequency and magnitude of high-ozone events are substantially greater in China. Key metrics include the fourth highest daily maximum 8-hour average ozone (4MDA8), the number of days exceeding 70 ppb (NDGT70), and cumulative exposure indices like SOMO35 (sum of ozone means over 35 ppb). Chinas warm-season 4MDA8 averages around 86 ppb, exceeding other regions by 630\%, while NDGT70 values are 93575\% higher, indicating more frequent episodes of elevated ozone. Vegetation exposure metrics such as AOT40 and W126, which correlate with ozone-induced plant damage, are also significantly elevated in China, suggesting greater risks to agricultural productivity and ecosystem health.

Spatially, ozone pollution hotspots in China are concentrated in densely populated and industrialized regions including the North China Plain, Yangtze River Delta, and Pearl River Delta, with some western areas affected due to topography and local emissions. Seasonal patterns show ozone peaks in late spring and early summer, influenced by regional meteorology such as the Asian summer monsoon, which modulates photochemical activity and pollutant transport.

Temporal analysis from 2013 to 2017 indicates a rising trend in ozone levels across Chinese cities, with annual increases in exposure metrics ranging from approximately 3.7\% to over 15\% per year. This contrasts with stable or declining ozone trends in Europe and the United States over recent decades. The increase in ozone occurs despite reductions in primary pollutants like SO2, NO2, CO, and fine particulate matter (PM2.5), reflecting complex photochemical interactions. In particular, reductions in NOx or PM2.5 can paradoxically enhance ozone formation in VOC-sensitive regimes prevalent in eastern China. Rising VOC emissions and meteorological factors such as hotter, drier summers also contribute to elevated ozone.

These findings highlight China as a current global hotspot for surface ozone pollution, with greater human and vegetation exposure than other industrialized regions with extensive monitoring. The severity and increasing trend of ozone pollution pose challenges for air quality management, indicating a need for targeted control strategies focusing on VOC emissions and comprehensive understanding of chemical and meteorological influences on ozone formation.

\textbf{\emph{\textcolor{DeepPurple}{Data Code}}}

\begin{lstlisting}
#!/usr/bin/env python3
# -*- coding: utf-8 -*-
"""
Paper: Severe Surface Ozone Pollution in China: A Global Perspective
Authors: Xiao Lu, Jiayun Hong, Lin Zhang, et al.
Year: 2018

Data generation script for simulating hourly surface ozone data.
Python Version: 3.10.12
"""

import sys

assert sys.version_info >= (3, 10), "This code requires Python 3.10 or higher"

# Dependencies
# pip install numpy==1.24.3 pandas==2.0.3

import numpy as np
import pandas as pd
from pathlib import Path
import os


def generate_hourly_ozone_data(
        n_sites: int,
        start_date: str,
        end_date: str,
        region_params: dict
) -> pd.DataFrame:
    """
    Generate synthetic hourly ozone data for multiple sites.
    Tag: [Simulation]

    Args:
        n_sites (int): The number of monitoring sites to simulate.
        start_date (str): The start date for the data series (e.g., '2013-01-01').
        end_date (str): The end date for the data series (e.g., '2017-12-31').
        region_params (dict): A dictionary containing parameters for the region.
            Keys should include 'base_mean', 'seasonal_amp', 'daily_amp',
            'noise_level', 'event_prob', 'event_strength'.

    Returns:
        pd.DataFrame: A DataFrame with columns ['site_id', 'timestamp', 'ozone_ppb'].

    Examples:
        >>> params = {
        ...     'base_mean': 40, 'seasonal_amp': 15, 'daily_amp': 20,
        ...     'noise_level': 5, 'event_prob': 0.02, 'event_strength': 40
        ... }
        >>> df = generate_hourly_ozone_data(2, '2017-01-01', '2017-01-31', params)
        >>> print(df.shape)
        (1488, 3)
    """
    np.random.seed(0+42)
    timestamps = pd.to_datetime(np.arange(
        np.datetime64(start_date),
        np.datetime64(end_date) + np.timedelta64(1, 'D'),
        np.timedelta64(1, 'h')
    ))
    n_hours = len(timestamps)

    # Prepare time feature vectors
    day_of_year = timestamps.dayofyear
    hour_of_day = timestamps.hour

    all_sites_data = []
    for site_id in range(n_sites):
        # Base signal = seasonal cycle + daily cycle
        seasonal_cycle = region_params['seasonal_amp'] * np.sin(2 * np.pi * (day_of_year - 90) / 365.25)
        daily_cycle = region_params['daily_amp'] * np.sin(2 * np.pi * (hour_of_day - 8) / 24)

        base_signal = region_params['base_mean'] + seasonal_cycle + daily_cycle

        # Add random noise
        noise = np.random.randn(n_hours) * region_params['noise_level']

        # Simulate high pollution events
        events = np.zeros(n_hours)
        for i in range(n_hours):
            if np.random.rand() < region_params['event_prob']:
                # Pollution event lasts 24-72 hours
                duration = np.random.randint(24, 73)
                event_end = min(i + duration, n_hours)
                event_shape = np.sin(np.linspace(0, np.pi, event_end - i))
                events[i:event_end] += region_params['event_strength'] * event_shape

        # Compose final signal
        ozone_concentration = base_signal + noise + events
        # Ensure concentration values are non-negative
        ozone_concentration = np.maximum(ozone_concentration, 0)

        site_df = pd.DataFrame({
            'site_id': f'site_{site_id}',
            'timestamp': timestamps,
            'ozone_ppb': ozone_concentration
        })
        all_sites_data.append(site_df)

    return pd.concat(all_sites_data, ignore_index=True)


def save_data_to_csv(df: pd.DataFrame, file_path: str):
    """
    Save a DataFrame to a CSV file.
    Tag: [Data saving]

    Args:
        df (pd.DataFrame): The DataFrame to save.
        file_path (str): The path to the output CSV file.

    Returns:
        None

    Examples:
        >>> data = pd.DataFrame({'col1': [1, 2], 'col2': [3, 4]})
        >>> save_data_to_csv(data, 'data/test.csv')
    """
    # Ensure directory exists
    output_dir = os.path.dirname(file_path)
    if not os.path.exists(output_dir):
        os.makedirs(output_dir)
    df.to_csv(file_path, index=False)
    print(f"Data has been saved to: {file_path}")


if __name__ == "__main__":
    # Set different parameters for China and JKEU regions according to the paper description
    # China region parameters: higher base value, stronger seasonal and daily variations, more frequent and stronger high pollution events
    china_params = {
        'base_mean': 45,
        'seasonal_amp': 20,
        'daily_amp': 25,
        'noise_level': 8,
        'event_prob': 0.015,  # Higher event occurrence probability
        'event_strength': 50  # Stronger event intensity
    }

    # JKEU region parameters: relatively moderate pollution levels
    jkeu_params = {
        'base_mean': 35,
        'seasonal_amp': 15,
        'daily_amp': 20,
        'noise_level': 5,
        'event_prob': 0.005,  # Lower event occurrence probability
        'event_strength': 30  # Weaker event intensity
    }

    # To reduce runtime, we only simulate one year of data
    START_DATE = '2017-01-01'
    END_DATE = '2017-12-31'
    NUM_SITES = 10  # Simulate 10 sites

    print("Generating simulated ozone data for China region...")
    china_ozone_data = generate_hourly_ozone_data(NUM_SITES, START_DATE, END_DATE, china_params)

    print("Generating simulated ozone data for JKEU region...")
    jkeu_ozone_data = generate_hourly_ozone_data(NUM_SITES, START_DATE, END_DATE, jkeu_params)

    # Create data directory and save files
    data_dir = Path("data")
    data_dir.mkdir(exist_ok=True)

    save_data_to_csv(china_ozone_data, str(data_dir / "china_ozone_data.csv"))
    save_data_to_csv(jkeu_ozone_data, str(data_dir / "jkeu_ozone_data.csv"))
\end{lstlisting}

\textbf{\emph{\textcolor{DeepPurple}{Main Code with Incomplete Functions}}}

\begin{lstlisting}
#!/usr/bin/env python3
# -*- coding: utf-8 -*-
"""
Paper: Severe Surface Ozone Pollution in China: A Global Perspective
Authors: Xiao Lu, Jiayun Hong, Lin Zhang, et al.
Year: 2018

Implementation of ozone pollution metrics calculation.
Python Version: 3.10.12
"""

import sys

assert sys.version_info >= (3, 10), "This code requires Python 3.10 or higher"

# Dependencies
# pip install numpy==1.24.3 pandas==2.0.3

import numpy as np
import pandas as pd


def load_ozone_data(file_path: str) -> pd.DataFrame:
    """
    Load hourly ozone data from a CSV file.
    Tag: [Data loading]

    Args:
        file_path (str): The path to the CSV data file.

    Returns:
        pd.DataFrame: A DataFrame with a datetime index and ozone data.

    Examples:
        >>> df = load_ozone_data('data/china_ozone_data.csv')
        >>> print(df.columns)
        Index(['site_id', 'ozone_ppb'], dtype='object')
    """
    df = pd.read_csv(file_path, parse_dates=['timestamp'])
    df = df.set_index('timestamp')
    return df


def calculate_mda8(daily_hourly_data: pd.Series) -> float:
    """
    Calculate the Daily Maximum 8-hour Average (MDA8) ozone concentration.
    Tag: [Numerical calculation]

    Args:
        daily_hourly_data (pd.Series): A Series of 24 hourly ozone values for a single day.

    Returns:
        float: The MDA8 value in ppb. Returns np.nan if data is insufficient.

    Examples:
        >>> hours = pd.to_datetime(pd.date_range('2023-07-01', periods=24, freq='h'))
        >>> data = pd.Series(np.sin(np.linspace(0, 2*np.pi, 24)) * 20 + 50, index=hours)
        >>> mda8 = calculate_mda8(data)
        >>> print(round(mda8, 2))
        67.68
    """
    pass # [Please complete the code]


def calculate_4mda8(mda8_series: pd.Series) -> float:
    """
    Calculate the 4th highest MDA8 value for a given period.
    Tag: [Numerical calculation]

    Args:
        mda8_series (pd.Series): A Series of daily MDA8 values.

    Returns:
        float: The 4th highest MDA8 value. Returns np.nan if data is insufficient.

    Examples:
        >>> data = pd.Series([80, 90, 70, 100, 110, 60])
        >>> val = calculate_4mda8(data)
        >>> print(val)
        80.0
    """
    valid_mda8 = mda8_series.dropna()
    if len(valid_mda8) < 4:
        return np.nan
    return valid_mda8.sort_values(ascending=False).iloc[3]


def calculate_ndgt70(mda8_series: pd.Series) -> int:
    """
    Calculate the total number of days with MDA8 values > 70 ppb.
    Tag: [Numerical calculation]

    Args:
        mda8_series (pd.Series): A Series of daily MDA8 values.

    Returns:
        int: The count of days where MDA8 > 70 ppb.

    Examples:
        >>> data = pd.Series([65, 71, 85, 70, 70.1])
        >>> count = calculate_ndgt70(data)
        >>> print(count)
        3
    """
    return (mda8_series > 70).sum()


def calculate_aot40(hourly_data: pd.Series) -> float:
    """
    Calculate the AOT40 (Accumulated Ozone over a Threshold of 40 ppb).
    Tag: [Numerical calculation]

    Args:
        hourly_data (pd.Series): A Series of hourly ozone data for the entire period.
                                 The function will filter for daytime hours (08:00-19:59).

    Returns:
        float: The total AOT40 value in ppb-hours.

    Examples:
        >>> hours = pd.to_datetime(pd.date_range('2023-07-01', periods=24, freq='h'))
        >>> data = pd.Series(np.arange(30, 54), index=hours)
        >>> aot40 = calculate_aot40(data)
        >>> print(aot40)
        91.0
    """
    daytime_data = hourly_data[(hourly_data.index.hour >= 8) & (hourly_data.index.hour <= 19)]
    # Calculate the portion exceeding 40 ppb each hour
    exceedances = np.maximum(0, daytime_data - 40)
    return exceedances.sum()


def calculate_w126(hourly_data: pd.Series) -> float:
    """
    Calculate the W126 metric, a weighted cumulative exposure index.
    Tag: [Numerical calculation]

    Args:
        hourly_data (pd.Series): A Series of hourly ozone data for the entire period.
                                 The function will filter for daytime hours (08:00-19:59).

    Returns:
        float: The total W126 value in ppb-hours.

    Examples:
        >>> hours = pd.to_datetime(pd.date_range('2023-07-01', periods=24, freq='h'))
        >>> data = pd.Series(np.full(24, 80), index=hours) # Constant 80 ppb
        >>> w126 = calculate_w126(data)
        >>> print(round(w126, 2))
        954.16
    """
    pass # [Please complete the code]


def analyze_regional_metrics(df: pd.DataFrame) -> dict:
    """
    Analyze and compute all key ozone metrics for a given region's data.
    Tag: [Statistical analysis]

    Args:
        df (pd.DataFrame): The DataFrame containing hourly ozone data for a region.

    Returns:
        dict: A dictionary of regionally-averaged ozone metrics.

    Examples:
        >>> df = load_ozone_data('data/china_ozone_data.csv')
        >>> metrics = analyze_regional_metrics(df)
        >>> print(metrics.keys())
        dict_keys(['avg_4mda8', 'avg_ndgt70', 'avg_aot40', 'avg_w126'])
    """
    site_metrics = []
    # Group by site for calculation
    for site_id, site_data in df.groupby('site_id'):
        # Filter warm season data (April-September)
        warm_season_data = site_data[(site_data.index.month >= 4) & (site_data.index.month <= 9)]

        # Calculate daily MDA8
        daily_mda8 = warm_season_data['ozone_ppb'].resample('D').apply(calculate_mda8).dropna()

        if daily_mda8.empty:
            continue

        # Calculate various metrics
        m4da8 = calculate_4mda8(daily_mda8)
        ndgt70 = calculate_ndgt70(daily_mda8)
        aot40 = calculate_aot40(warm_season_data['ozone_ppb'])
        w126 = calculate_w126(warm_season_data['ozone_ppb'])

        site_metrics.append({
            'site_id': site_id,
            '4mda8': m4da8,
            'ndgt70': ndgt70,
            'aot40': aot40,
            'w126': w126
        })

    # Calculate regional averages
    metrics_df = pd.DataFrame(site_metrics).dropna()
    if metrics_df.empty:
        return {
            'avg_4mda8': 0, 'avg_ndgt70': 0, 'avg_aot40': 0, 'avg_w126': 0
        }

    regional_avg = {
        'avg_4mda8': metrics_df['4mda8'].mean(),
        'avg_ndgt70': metrics_df['ndgt70'].mean(),
        'avg_aot40': metrics_df['aot40'].mean(),
        'avg_w126': metrics_df['w126'].mean()
    }
    return regional_avg


if __name__ == "__main__":
    # Load data
    try:
        china_df = load_ozone_data('data/china_ozone_data.csv')
        jkeu_df = load_ozone_data('data/jkeu_ozone_data.csv')
    except FileNotFoundError:
        print("Error: Data file not found. Please run data.py to generate the data first.")
        sys.exit(1)

    print("Analyzing China region data...")
    china_metrics = analyze_regional_metrics(china_df)

    print("Analyzing JKEU region data...")
    jkeu_metrics = analyze_regional_metrics(jkeu_df)

    # Display results comparison in text format
    print("\n" + "=" * 60)
    print("             Regional Comparison of Ozone Pollution Metrics (Warm Season Average)")
    print("=" * 60)
    print(f"{'Metric':<20} | {'China':>15} | {'JKEU':>15}")
    print("-" * 60)
    print(f"{'4th Highest MDA8 (ppb)':<20} | {china_metrics['avg_4mda8']:>15.2f} | {jkeu_metrics['avg_4mda8']:>15.2f}")
    print(f"{'NDGT70 (days)':<20} | {china_metrics['avg_ndgt70']:>15.2f} | {jkeu_metrics['avg_ndgt70']:>15.2f}")
    print(f"{'AOT40 (ppb-h)':<20} | {china_metrics['avg_aot40']:>15.2f} | {jkeu_metrics['avg_aot40']:>15.2f}")
    print(f"{'W126 (ppb-h)':<20} | {china_metrics['avg_w126']:>15.2f} | {jkeu_metrics['avg_w126']:>15.2f}")
    print("=" * 60)

    # Calculate final output: ratio of China's NDGT70 metric relative to JKEU
    # Add numerical stability check
    epsilon = 1e-8
    ndgt70_ratio = china_metrics['avg_ndgt70'] / (jkeu_metrics['avg_ndgt70'] + epsilon)

    print("\nConclusion: Simulation results show that the frequency of high ozone pollution events (NDGT70)")
    print(f"in China is approximately {ndgt70_ratio:.2f} times that of the JKEU region, consistent with the trend found in the original paper.")

    print("[Final Output]")
    print(ndgt70_ratio)
\end{lstlisting}

\textbf{\emph{\textcolor{DeepPurple}{Answer}}}

\begin{lstlisting}
def calculate_w126(hourly_data: pd.Series) -> float:
    """
    Calculate the W126 metric, a weighted cumulative exposure index.
    Tag: [Numerical calculation]

    Args:
        hourly_data (pd.Series): A Series of hourly ozone data for the entire period.
                                 The function will filter for daytime hours (08:00-19:59).

    Returns:
        float: The total W126 value in ppb-hours.

    Examples:
        >>> hours = pd.to_datetime(pd.date_range('2023-07-01', periods=24, freq='h'))
        >>> data = pd.Series(np.full(24, 80), index=hours) # Constant 80 ppb
        >>> w126 = calculate_w126(data)
        >>> print(round(w126, 2))
        954.16
    """
    epsilon = 1e-8
    daytime_data = hourly_data[(hourly_data.index.hour >= 8) & (hourly_data.index.hour <= 19)]

    # W126 weight function parameters
    M = 4403
    A = 126

    # Calculate weights
    # Using np.exp with negative input is usually safe, but epsilon is added to denominator
    weights = 1 / (1 + M * np.exp(-A * daytime_data / 1000) + epsilon)

    # Calculate weighted concentration and sum
    w126 = (weights * daytime_data).sum()
    return w126

def calculate_mda8(daily_hourly_data: pd.Series) -> float:
    """
    Calculate the Daily Maximum 8-hour Average (MDA8) ozone concentration.
    Tag: [Numerical calculation]

    Args:
        daily_hourly_data (pd.Series): A Series of 24 hourly ozone values for a single day.

    Returns:
        float: The MDA8 value in ppb. Returns np.nan if data is insufficient.

    Examples:
        >>> hours = pd.to_datetime(pd.date_range('2023-07-01', periods=24, freq='h'))
        >>> data = pd.Series(np.sin(np.linspace(0, 2*np.pi, 24)) * 20 + 50, index=hours)
        >>> mda8 = calculate_mda8(data)
        >>> print(round(mda8, 2))
        67.68
    """
    # At least 18 (75%) hours of data are required to calculate the 8-hour average
    if daily_hourly_data.count() < 18:
        return np.nan
    # Calculate 8-hour rolling average
    rolling_8hr_mean = daily_hourly_data.rolling(window=8, min_periods=6).mean()
    if rolling_8hr_mean.empty or rolling_8hr_mean.isnull().all():
        return np.nan
    return rolling_8hr_mean.max()
\end{lstlisting}

\end{tcolorbox}
%-----------------------------------------------------------%-----------------------------------------------------------
